An aerodynamic measurement system to improve the efficiency of wind turbine rotor blades

The wind energy sector is growing rapidly with the installation of wind turbines with long, slender blades in a diverse range of locations. To enhance the operational performance under specific wind conditions and to validate the aerodynamic design of flexible blades, it is crucial to obtain comprehensive data on the aerodynamic behaviour of the blades in the field, such as time-resolved pressure distributions, local inflow conditions and dynamic responses of the blade. However, published field measurements are scarce for large-scale rotor blades due to the complex and costly installation of the requisite measurement systems. In recent work, we developed a wireless and self-sufficient aerodynamic measurement system, named Aerosense, which is less complex and costly than conventional aerodynamic measurement systems. The Aerosense system uses Micro-Electro-Mechanical Systems (MEMS) sensors to obtain local aerodynamic pressures, blade motions, and inflow conditions. In this paper, we demonstrate the value of Aerosense in understanding the aerodynamic behaviour of rotor blades, using a 7kW wind turbine operating in the field. After a thorough calibration and correction process, we demonstrate, for example, that the pressure distribution can vary significantly during one rotation of the blade, even under stable wind conditions. These variations are found to be due to the misalignment of the wind direction with the wind turbine's rotational axis. We therefore conclude that the Aerosense measurement system is valuable for understanding the aerodynamic loading on rotor blades as well as the influence of the inflow conditions on wind turbine performance.

==> figures/latex/tikzset.tex <==
%*******************************************************
% tikz
%*******************************************************
\pgfkeys{/pgf/number format/.cd,precision=3, fixed} %zerofill

\pgfplotsset{every axis/.append style={
	view={0}{90}, scale only axis, axis on top,
	line width=0.1pt, tick style={line width=0.2pt},
	unbounded coords=jump, ylabel near ticks,
}}
\pgfplotsset{every axis plot/.append style={
	line width=1pt
}}
\pgfplotsset{every tick/.append style={
	color=black, major tick length=4pt
}}
\pgfplotsset{every outer axis line/.append style={-stealth}}

\pgfplotsset{every axis legend/.append style={
	at={(1,1)}, anchor=north east, inner sep=4pt, cells={anchor=east}, draw=none, fill=none, xshift=-1pt, yshift=-1pt
}}

\pgfplotsset{tick label style={font=\small},label style={font=\small},legend style={font=\small}, colorbar style={font=\scriptsize}}
%was font=\small before

\pgfplotsset{
    every non boxed y axis/.style={
    	ytick align=center,
        enlarge y limits=false,
        y axis line style={-},
},
    every boxed y axis/.style={},
}

\tikzset{subplotnr/.style={anchor=north west, xshift=2mm, yshift=-2mm, fill=none}}


\pgfplotsset{vaxis/.style={scale only axis, view={0}{90}, axis equal image, width=7cm, xmin=-0.26, xmax=0.76, ymin=-0.05, ymax=0.53, xlabel=$x/c$, xtick={-0.25,0,...,1}, ylabel=$z/c$, ytick={0,0.1,0.2,0.3,0.4,0.5}, axis on top}}

\pgfplotsset{minicolorbar/.style={point meta min=-0.04, point meta max=0.04, colormap name=kmap, colorbar horizontal, colorbar style={anchor=north west, at={($(current axis.north west)+(5mm,-0.5mm)$)}, width=0.23*\pgfkeysvalueof{/pgfplots/parent axis width}, height=0.2cm, scaled ticks=false, font=\tiny, xtick={-0.04,0,0.04}, title={\tiny $\omega c/\U_0$}, title style={at={(0.5,-2.4)}, anchor=north}}}}

\pgfplotsset{
    smarks/.style={only marks, mark=o, mark size=3, line width=0.7, error bars/.cd, y dir= both, y explicit,}, 
    smarks_r/.style={only marks, mark=x, mark size=4, error bars/.cd, y dir= both, y explicit,}, 
    %mark=*, mark size=1.5pt, mark options={solid,fill=gray},line width=0.8pt},
}

\pgfplotsset{
    colormap={TealGold}{
        rgb255(0.00pt)=(44,140,139); %1  -1 
        rgb255(55.56pt)=(51,143,132); %2 
        rgb255(111.11pt)=(58,146,126); %3
        rgb255(166.67pt)=(65,149,120); %4
        rgb255(222.22pt)=(73,153,114); %5  -2
        rgb255(277.78pt)=(80,156,107); %6 
        rgb255(333.33pt)=(87,159,101); %7
        rgb255(388.89pt)=(95,163,95); %8  
        rgb255(444.44pt)=(102,166,89); %9 -3
        rgb255(500.00pt)=(114,167,83); %10
        rgb255(555.56pt)=(130,167,77);  %11
        rgb255(611.11pt)=(146,166,71); %12
        rgb255(666.67pt)=(161,165,66); %13  
        rgb255(722.22pt)=(178,165,60);  %14 -4
        rgb255(777.78pt)=(194,164,54); %15
        rgb255(833.33pt)=(210,164,49); %16
        rgb255(888.89pt)=(226,163,43); %17
        rgb255(944.44pt)=(242,163,38); %18  -5
    }
}
\pgfplotsset{
    colormap={TealGoldDiv}{
        rgb255(0.00pt)=(44,140,139);
        rgb255(55.56pt)=(62,146,145);
        rgb255(111.11pt)=(80,153,152);
        rgb255(166.67pt)=(98,160,159);
        rgb255(222.22pt)=(116,167,166);
        rgb255(277.78pt)=(134,174,173);
        rgb255(333.33pt)=(152,180,180);
        rgb255(388.89pt)=(170,187,187);
        rgb255(444.44pt)=(188,194,194);
        rgb255(500.00pt)=(200,195,188);
        rgb255(555.56pt)=(205,191,169);
        rgb255(611.11pt)=(210,187,150);
        rgb255(666.67pt)=(216,183,132);
        rgb255(722.22pt)=(221,179,113);
        rgb255(777.78pt)=(226,175,94);
        rgb255(833.33pt)=(231,171,75);
        rgb255(888.89pt)=(236,167,56);
        rgb255(944.44pt)=(242,163,38);
    }
}

\pgfplotsset{
colormap={TealGoldCycle}{
    rgb255(0.00pt)=(44,140,139);
    rgb255(27.78pt)=(60,146,145);
    rgb255(55.56pt)=(77,152,151);
    rgb255(83.33pt)=(94,159,158);
    rgb255(111.11pt)=(114,166,165);
    rgb255(138.89pt)=(130,172,172);
    rgb255(166.67pt)=(147,179,178);
    rgb255(194.44pt)=(167,186,186);
    rgb255(222.22pt)=(184,192,192);
    rgb255(250.00pt)=(198,197,194);
    rgb255(277.78pt)=(204,192,174);
    rgb255(305.56pt)=(209,189,157);
    rgb255(333.33pt)=(214,185,139);
    rgb255(361.11pt)=(219,180,119);
    rgb255(388.89pt)=(224,177,102);
    rgb255(416.67pt)=(229,173,84);
    rgb255(444.44pt)=(234,168,64);
    rgb255(472.22pt)=(239,164,46);
    rgb255(500.00pt)=(237,165,43);
    rgb255(527.78pt)=(227,171,53);
    rgb255(555.56pt)=(216,177,64);
    rgb255(583.33pt)=(206,183,74);
    rgb255(611.11pt)=(196,189,84);
    rgb255(638.89pt)=(185,195,96);
    rgb255(666.67pt)=(175,201,106);
    rgb255(694.44pt)=(165,206,116);
    rgb255(722.22pt)=(154,213,128);
    rgb255(750.00pt)=(143,207,130);
    rgb255(777.78pt)=(131,199,131);
    rgb255(805.56pt)=(117,189,132);
    rgb255(833.33pt)=(105,181,133);
    rgb255(861.11pt)=(93,173,134);
    rgb255(888.89pt)=(79,164,136);
    rgb255(916.67pt)=(67,156,137);
    rgb255(944.44pt)=(55,148,138);
    rgb255(972.22pt)=(44,140,139);
}
}

\tikzset{mystyle/.style n args=2{fill=gray!50!black, opacity=0.7, circle, scale=1.2, pin={[pin distance=4mm, pin edge={gray!50!black,-,line width=0.8pt}, black!50!black, inner sep=0.6pt]#2:{\textbf{\normalsize #1}}}, inner sep=1.2pt}}
\tikzset{mystyledist/.style n args=3{fill=gray!50!black, opacity=0.7, circle, scale=1.2, pin={[pin distance=#3, pin edge={gray!50!black,-,line width=0.8pt}, black!50!black, inner sep=0.6pt]#2:{\textbf{\normalsize #1}}}, inner sep=1.2pt}}
\tikzset{styleKulites/.style={only marks, mark size=3pt,mark=*,draw=black,line width=0.1pt,fill opacity=0.6,draw opacity=0.6}}



\pgfplotsset{ymissing/.style={ylabel={}, yticklabels={}}}
\pgfplotsset{xmissing/.style={xlabel={}, xticklabels={}}}
\pgfplotsset{yaxisright/.append style={yticklabel pos=right,  ylabel near ticks, y label style={rotate=180}}}
\pgfplotsset{xaxistop/.append style={xticklabel pos=top,  xlabel near ticks, xlabel style={yshift=-0.5ex}}} %, axis x line*=top

\pgfplotsset{multyaxesright/.style n args={2}{
axis y line*=right,
every outer y axis line/.style={xshift=#1cm, #2, line width=0.2pt},
every tick/.style={xshift=#1cm, #2},
every y tick label/.append style={xshift=#1cm, #2},
y label style={#2, rotate=180}
}} % usage: multyaxesright={0}{royalblue}

\pgfplotsset{multyaxesleft/.style n args={2}{
axis y line*=left,
every outer y axis line/.style={xshift=#1cm, #2, line width=0.2pt},
every tick/.style={xshift=#1cm, #2},
every y tick label/.append style={xshift=#1cm, #2},
y label style={#2, rotate=0}
}}

\pgfplotsset{multxaxes/.style n args={3}{
axis x line*=#3,
every outer x axis line/.style={yshift=#1cm, #2, line width=0.2pt},
every tick/.style={yshift=#1cm, #2},
every x tick label/.append style={yshift=#1cm, #2},
x label style={#2}
}}

\tikzset{pics/carc/.style args={#1:#2:#3}{% clockwise
code={\draw[pic actions] (#1:#3) arc(#1:#2:#3) -- ++(#2-100:2mm);}}}
\tikzset{pics/ccarc/.style args={#1:#2:#3}{% counterclock
code={\draw[pic actions] (#1:#3) arc(#1:#2:#3) -- ++(#2+100:2mm);}}}

% ---- files loaded --------------------------------------------
% \pgfplotstableread{../datfiles/df_baros_zeroed_csv.dat}{\ZeroedPressure}


